Ego-GNNs: Exploiting Ego Structures in Graph Neural Networks

Graph neural networks (GNNs) have achieved remarkable success as a framework for deep learning on graph-structured data. However, GNNs are fundamentally limited by their tree-structured inductive bias: the WL-subtree kernel formulation bounds the representational capacity of GNNs, and polynomial-time GNNs are provably incapable of recognizing triangles in a graph. In this work, we propose to augment the GNN message-passing operations with information defined on ego graphs (i.e., the induced subgraph surrounding each node). We term these approaches Ego-GNNs and show that Ego-GNNs are provably more powerful than standard message-passing GNNs. In particular, we show that Ego-GNNs are capable of recognizing closed triangles, which is essential given the prominence of transitivity in real-world graphs. We also motivate our approach from the perspective of graph signal processing as a form of multiplex graph convolution. Experimental results on node classification using synthetic and real data highlight the achievable performance gains using this approach.

==> sections/old_proposed.tex <==
\section{Proposed Approach}


Our key proposal is to design a GNN algorithm that can naturally exploit the ego-structure of graphs. In doing so, we hope to improve the theoretical capacity of the model. In addition to that, we hope to potentially address known empirical limitations, such as the {\em over-smoothing} problem that results from node signals becoming uninformative after several rounds of GNNs message passing. 

Our approach involves performing message passing over the ego-graphs of all the nodes in a graph, rather than simply over the graph itself. 
% The node representation of node $i$ in a regular GNN with $K$ layers is an aggregation of messages traveling up a $K$-deep tree rooted at $i$ whose depth and breadth increases with each new layer. On the other hand, the same representation of node $i$ in an ego-graph oriented model would be an aggregation of messages traveling only within all of the ego-graphs containing node $i$.
In the following section, we will formalize how to construct a model that has this desired behavior using a graph  which is defined by a set of vertices $V$, an adjacency matrix $A$, and a matrix of node features $X$ which is defined as having size $|V| \times f$.

\subsection{Conceptual Motivation}

One way of motivating our Ego-GNN approach is based on the idea of message-passing over a {\em multiplex graph} defined over the original graph. 
In particular, we can construct a multiplex graph in which each layer of the multiplex corresponds to a particular ego-graph of the original graph, and the inter-layer connections are based on the original adjacency structure.
Message-passing on such a multiplex would involve passing messages between nodes in the same ego-graph (via the {\em intra-layer} edges), while also propagating information between ego-structures (via the {\em inter-layer} edges).  

% Formally, We define the multiplex ego-graph $\tilde{G}$ using a {\em supra-adjacency} matrix, $\tilde{A} \in \mathbb{R}^{|V|^2 \times |V|^2}$ constructed from the original graph $G$ as follows:
Formally, we can define a $|V|^2 \times |V|^2$ {\em supra-adjacency} matrix, $\tilde{A}$ constructed from the original graph $G$ as follows:
In particular, we can define the supra-adjacency matrix $\tilde{A}$ as follows:
\begin{equation}\label{eq:supra}
    \tilde{A} = \bigoplus_{i=1}^{|V|}A_i + (A \otimes I).
\end{equation}
Here, we are creating the {\em intra-layer} adjacency structure by taking the direct sum of matrices $A_i$, where each $A_i$ correspond to the $|V| \times |V|$ adjacency matrix of the $i$th ego-graph:
\begin{equation}
     \bigoplus_{i=1}^{|V|}A_i = \begin{pmatrix} A_1 & {} & {} & {} \\ {} & A_2 & {} & {} \\ {} & {} & \ddots & {} \\ {} & {} & {} & A_{|V|} \\ \end{pmatrix},
\end{equation}
where the off-diagonal blocks are zero. 
The term $(A \otimes I)$ in Equation \eqref{eq:supra} defines the {\em inter-layer} adjacency structure and is created based on the Kronecker product between the original adjacency matrix and the identity. 
Intuitively, the intra-layer diagonal blocks correspond to each ego-graph, and the off-diagonal blocks connect two ego-graphs if they share a node (i.e., if the corresponding nodes are connected in the original graph). 

Our approach's core idea is to perform a message passing over $\tilde{A}$ rather than the original graph.
However, of course, naively implementing a GNN on the $|V|^2 \times |V|^2$ matrix $\tilde{A}$ would be computationally expensive with the quadratic increase in the size of graph. 
Thus, in the following sections, we describe incremental relaxations and refinements that allow us to implement our Ego-GNN approach in a tractable manner.

\subsection{Sequencing the Intra- and Inter-layer Messages}

In this section, we describe how we approximate message-passing over the full multiplex, defined by the supra-adjacency matrix $\tilde{A}$, using a sequential approach where we run the intra-layer (i.e., within ego-graph) and inter-layer (i.e., between ego-graph) operations in sequence. 
Note also that we assume that our goal is to maintain a single representation $H[i] \in \mathbb{R}^f$ for each node in the graph, and we will use the notation $H_{(t)} \in \mathbb{R}^{|V| \times f}$ to denote the matrix of node representations at layer $t$ of the model. 

\xhdr{Message-passing within ego-graphs}
We first run message-passing independently within each ego-graph. 
To do so, we tile the node representations vertically $|V|$ times before the matrix multiplication:
\[
    \hat{H}_{(t-1)} = \begin{pmatrix} H_{(t-1)} \\ \vdots \\ H_{(t-1)} \end{pmatrix}, \: \hat{H}_{(t-1)} \! \in \mathbb{R}^{|V|^2 \times f}
\]
Multiplying this tiled representation by a power of intra-layer portion of the supra-adacency matrix, we get 
\begin{equation}
    \hat{H}_{(t)} = \left(\bigoplus_{i=1}^{|V|}A_i\right)^p\hat{H}_{(t-1)} \label{eq:2},
\end{equation}
where $p$ is the desired scale of the message-passing within each ego-graph (e.g., $p=2$ corresponds to aggregating over two-hop neighborhoods in the ego-graphs). 

\xhdr{Aggregating across ego-graphs}
After Equation \ref{eq:2}, $\hat{H}_{(t)} \in \mathbb{R}^{|V|^2 \times f}$ contains the representation of every node in every ego-graph.
We therefore need to aggregate information across the different ego-graphs in order to collapse it back into a $|V| \times f$ matrix. 

In our conceptual motivation, we envisioned connected ego-graph layers in the supra-adjacency matrix based on the original adjacency structure of the graph. 
In intuitive terms, we would like the overall representation of each node to depend on its representation in each ego-graph to which it belongs. 
With this in mind, a natural way to approximate the {\em inter-layer} message-passing of the full multiplex is to define each node $i$'s representation in our final matrix $H[i]_{(t)}$ as the average of that node's representation in all of the ego-graphs that contain it. We therefore define each row of $H_{(t)}$ as follows:
\begin{equation}
    H[i]_{(t)} = \frac{ \displaystyle\sum_{j \in Ego(i)}^{} \hat{H}_{(t)}[(j - 1)|V| + i] }{|Ego(i)|} \label{eq:3}
\end{equation}
Where $Ego(i)$ is the list of all the nodes whose ego-graphs contain node $i$.

This approach based on sequencing the within-ego-graph and between-ego-graph operations is sound and would produce the desired node representations that leverage the ego-structure of the graph. 
However, it as two major flaws. Firstly, it is memory-intensive due to the fact that $\hat{H}_{(t)}$ cannot be stored using a sparse matrix. Second, the method has not been properly normalized, which can lead to stability issues. 

\subsection{The Ego-GNN Model}

In this section, we build upon the sequential approach proposed above and remedy its key limitations to describe our full Ego-GNN approach. 

\xhdr{Addressing the memory limitations}
The memory problem caused by $\hat{H}_{(t)}$ can be solved by performing the within-ego-graph operations in an iterative manner rather than all at once. 
In particular, instead of carrying out Equation \eqref{eq:2}, we do a combination of operations which calculates $H_{(t)}$ without ever needing to go through $\hat{H}_{(t)}$. These operations are captured in the following sum, which is equivalent to Equation \eqref{eq:3}:
\begin{equation}
    H[i]_{(t)} = \frac{ \left( \displaystyle\sum_{j = 1}^{|V|} A_j^p H_{(t-1)}  \right) [i]   }{|Ego(i)|} \label{eq:4}
\end{equation}
%The reason this sum is almost equivalent is precisely because of the way we define the adjacency matrices $A_i$ of each ego-graph. They are each $|V| \times |V|$ matrices which means that the nodes not included in the ego-graph will be represented by rows and columns of zeros. This means that the $i$th row of the sum in Equation \eqref{eq:4} is equal to the sum in Equation \eqref{eq:3} for node $i$. Therefore, Equation \eqref{eq:4} is sound and solves the memory issue caused by $\hat{H}_{(i)}$. The only way that this representation differs is its inability to capture the relationships represented by the off diagonal blocks  of $\tilde{A}$, but this can be accounted for by feeding the result of Equation \eqref{eq:4} into a conventional message-passing layer. This works because the off diagonal blocks in $\tilde{A}$ represent edges between ego-graphs, which together simply make up the adjacency matrix of the original graph.

\xhdr{Adding normalization}
Finally, we only need to apply an appropriate normalization to the model to improve its performance further. 
For generality, we assume that each ego-adjacency matrix $A_i$ can be replaced by an appropriately normalized counter-part $\hat{A}_i$ (e.g., the popular symmetric normalization $\hat{A}_i = D_i^{-\frac{1}{2}}A_iD_i^{-\frac{1}{2}}$, where $D_i$ is diagonal degree matrix of $A_i$).

\xhdr{Putting it all together}
Mixing all of these concepts together along with the fact that $|Ego(i)|$ is equal to $deg(i) + 1$, we can formulate the entire Ego-GNN model with one equation:
\begin{equation}
    H[i]_{(t)} = \frac{ \left( \displaystyle\sum_{j = 1}^{|V|} \hat{A}_j^p H_{(t-1)}  \right) [i]   }{deg(i) + 1} \label{eq:5}
\end{equation}

\xhdr{Interleaving with standard GNN layers}
Finally, we note that the ego-message passing in Equation \ref{eq:5} can be interleaved with layers of standard GNN message-passing, such as the simple propagation rule proposed in \cite{kipf2016semi}.
%Where $\hat{A}_j$ can equal the normalized adjacency matrix of ego-graph $j$ or the unchanged adjacency matrix of ego-graph $j$ depending on the needs of the task. Opting for a normalized adjacency matrix would entail using the following formula:
%\[
 %   \hat{A}_j = D_j^{-1/2} A_j D_j^{-1/2}
%\]
%Where $D_j$ is the diagonal degree matrix of the ego-graph of node $i$.

%When integrated into a model, the Ego-GNN layer must always be followed by a conventional message-passing layer to account for the missing off diagonal blocks of $\tilde{A}$ introduced in Equation \eqref{eq:1}.

==> sections/old_theoretical_motive.tex <==
\section{Theoretical Motivations}

We briefly remark on some of the theoretical motivations behind the Ego-GNN approach, both in terms of counting closed triangles as well as motivations from graph signal processing. 

\xhdr{Ego-GNNs and closed triangles}
First, we can note that Ego-GNN layers can be trivially used to recognize the existence of closed triangles in a graph.
For example, assuming constant features as node inputs, counting triangles can be performed via two rounds of message-passing in the ego-graphs: one round to compute node degrees and a second round for the central node to count the degree of each of its neighbors in the ego-graph. 
This simple approach suffices due to the fact that the number of closed triangles in a node's neighborhood is directly computable from the degrees of the nodes in its ego-graph. 
Note, however, that this does not guarantee that an Ego-GNN will learn such a function easily from data. 

\xhdr{Ego-GNNs and the classical WL Test}
One important facet of Ego-GNNs is that they are provably more powerful than the classical WL test (in other words, they can produce distinct labels of graphs normally given identical labels using the standard WL test algorithm). We can show this by manually calculating the labels generated by an Ego-GNN on a set of simple graphs known to be mislabeled by the regular WL test. In this case, we will use $C_6$, the cycle graph of length $6$, and $2C_3$, a graph consisting of two disjoint $3$-cycles, and set the features of all of the nodes in both graphs to be the same:

\includegraphics[width=0.47\textwidth, height=3.9cm]{Ego-Comparison.png}

\includegraphics[width=0.47\textwidth, height=2.1cm]{Ego-Computation.png}

\[
X_{(C_6)}[i] = X_{(2C_3)}[i] = [1, 1, 1] \quad \text{for all } i \text{ in } (1 ... 6)
\]
%\[
%X_{(C_6)} = X_{(2C_3)} = \begin{bmatrix} 1 & 1 & 1\\1 & 1 & 1\\1 & 1 & 1\\1 & 1 & 1\\1 & 1 & 1\\1 & 1 & 1 \end{bmatrix}
%\]
We will begin with $C_6$. First we will use Equation \eqref{eq:5} to calculate $H_{C_6}$. We will set $p$ to $1$ for this derivation:
%\[
%\displaystyle\sum_{j = 1}^{6} (A_{C_6})_{j} (X_{C_6}) = \begin{bmatrix} 7 & 7 & 7\\7 & 7 & 7\\7 & 7 & 7\\7 & 7 & 7\\7 & 7 & 7\\7 & 7 & 7 \end{bmatrix}
%\]
%\[
%\displaystyle\sum_{j = 1}^{6} (A_{2C_3})_{j} (X_{2C_3}) = \begin{bmatrix} 9 & 9 & 9\\9 & 9 & 9\\9 & 9 & 9\\9 & 9 & 9\\9 & 9 & 9\\9 & 9 & 9 \end{bmatrix}
%\]
\[
\frac{\left( \displaystyle\sum_{j = 1}^{6} (A_{C_6})_{j} (X_{C_6}) \right)[i]}{deg(i) + 1} = [2.\overline{3}, 2.\overline{3}, 2.\overline{3}] \quad \text{for all } i \text{ in } (1 ... 6)
\]
%\[
%\left( \displaystyle\sum_{j = 1}^{6} (A_{2C_3})_{j} (X_{2C_3}) \right)[i] = [9, 9, 9] \quad \text{for all } i \text{ in } (1 ... 6)
%\]
We then interleave the result with a normal message-passing aggregation layer to get the final node labels of $C_6$:
%\[
%A_{C_6} \left( \frac{\left( \displaystyle\sum_{j = 1}^{6} (A_{C_6})_{j} (X_{C_6}) \right)[i]}{deg(i) + 1} \right) = [7, 7, 7] \quad \text{for all } i \text{ in } (1 ... 6)
%\]
\[
(A_{C_6} H_{C_6})[i]  = [7, 7, 7] \quad \text{for all } i \text{ in } (1 ... 6)
\]
The aggregated graph representation can then simply be the average of all of the node labels, making the representation of $C_6$ equal to $[7, 7, 7]$. By using the exact same process for $2C_3$, and replacing the appropriate adjacency matrix and ego-adjacency matrices, we get the following result:
\[
(A_{2C_3} H_{2C_3})[i]  = [9, 9, 9] \quad \text{for all } i \text{ in } (1 ... 6)
\]
This means our representation of $2C_3$ is $[9, 9, 9]$, which is not equal to the representation of $C_6$, meaning that Ego-GNNs are capable of distinguishing between the two graphs. \\
For clarity, we can easily show that regular message passing does not yield this powerful result. Let us run a $2$-layer message-passing aggregation to show this:
\[
(A_{C_6}^2 X_{C_6})[i] = (A_{2C_3}^2 X_{2C_3})[i] = [9, 9, 9] \quad \text{for all } i \text{ in } (1 ... 6)
\]
As we expected, standard message-passing is not capable of beating the classical WL test with regards to graph discrimination, while Ego-GNNs can achieve this. \\

\xhdr{Ego-GNNs and graph convolutions}
Ego-GNNs can also be motivated as a graph convolution on the multiplex graph defined by Equation \eqref{eq:supra}. Interestingly, based on the multiplex networks theory, we know that the spectrum of this multiplex graph has a close relationship to the original graph. In particular, based on the perturbation analysis of Sole et al. \cite{sole2013spectral}, we know that there are natural conditions under which the spectrum of this multiplex contains frequencies corresponding to the original graph (via the inter-layer structure) as well as frequencies from the ego-graphs (via the intra-layer structure). 
Moreover, based on the fact that the ego-graphs are all subgraphs of the original graph, the well-known eigenvalue interlacing theorem \cite{chung1997spectral} implies that intra-layer frequencies will interlace the original graph spectrum. This suggests that the Ego-GNN approach can be motivated as a way to give access to a broader set of meaningful frequencies over which to perform graph convolutions. 

